Semi-Supervised Medical Image Segmentation via Cross Teaching between CNN and Transformer

Recently, deep learning with Convolutional Neural Networks (CNNs) and Transformers has shown encouraging results in fully supervised medical image segmentation. However, it is still challenging for them to achieve good performance with limited annotations for training. In this work, we present a very simple yet efficient framework for semi-supervised medical image segmentation by introducing the cross teaching between CNN and Transformer. Specifically, we simplify the classical deep co-training from consistency regularization to cross teaching, where the prediction of a network is used as the pseudo label to supervise the other network directly end-to-end. Considering the difference in learning paradigm between CNN and Transformer, we introduce the Cross Teaching between CNN and Transformer rather than just using CNNs. Experiments on a public benchmark show that our method outperforms eight existing semi-supervised learning methods just with a simpler framework. Notably, this work may be the first attempt to combine CNN and transformer for semi-supervised medical image segmentation and achieve promising results on a public benchmark. The code will be released at: https://github.com/HiLab-git/SSL4MIS.

==> hacks/many-authors-hack.tex <==
%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}
